Accelerating Ill-Conditioned Low-Rank Matrix Estimation via Scaled Gradient Descent

Low-rank matrix estimation is a canonical problem that finds numerous applications in signal processing, machine learning and imaging science. A popular approach in practice is to factorize the matrix into two compact low-rank factors, and then optimize these factors directly via simple iterative methods such as gradient descent and alternating minimization. Despite nonconvexity, recent literatures have shown that these simple heuristics in fact achieve linear convergence when initialized properly for a growing number of problems of interest. However, upon closer examination, existing approaches can still be computationally expensive especially for ill-conditioned matrices: the convergence rate of gradient descent depends linearly on the condition number of the low-rank matrix, while the per-iteration cost of alternating minimization is often prohibitive for large matrices. The goal of this paper is to set forth a competitive algorithmic approach dubbed Scaled Gradient Descent (ScaledGD) which can be viewed as pre-conditioned or diagonally-scaled gradient descent, where the pre-conditioners are adaptive and iteration-varying with a minimal computational overhead. With tailored variants for low-rank matrix sensing, robust principal component analysis and matrix completion, we theoretically show that ScaledGD achieves the best of both worlds: it converges linearly at a rate independent of the condition number of the low-rank matrix similar as alternating minimization, while maintaining the low per-iteration cost of gradient descent. Our analysis is also applicable to general loss functions that are restricted strongly convex and smooth over low-rank matrices. To the best of our knowledge, ScaledGD is the first algorithm that provably has such properties over a wide range of low-rank matrix estimation tasks.

==> main-results.tex <==

\section{Theoretical Guarantees}\label{sec:main-results}

This section is devoted to formally establishing the statistical and computational guarantees of \texttt{ScaledGD}. We start with necessary notations. Denote by $\bU_{\star}\bSigma_{\star}\bV_{\star}^{\top}$ the compact singular value decomposition (SVD) of the rank-$r$ matrix $\bX_{\star}\in\RR^{n_{1}\times n_{2}}$, i.e.~$\bX_{\star}=\bU_{\star}\bSigma_{\star}\bV_{\star}^{\top}$.
Here $\bU_{\star}\in\RR^{n_{1}\times r}$ and $\bV_{\star}\in\RR^{n_{2}\times r}$ are composed of $r$ left and right singular vectors, respectively, and $\bSigma_{\star}\in\RR^{r\times r}$ is a diagonal matrix consisting of $r$ singular values of $\bX_{\star}$ organized in a non-increasing order, i.e.~$\sigma_{1}(\bX_{\star})\ge\dots\ge\sigma_{r}(\bX_{\star})>0$. Define 
\begin{align}
\kappa\coloneqq\sigma_{1}(\bX_{\star})/\sigma_{r}(\bX_{\star})\label{eq:kappa}
\end{align} 
as the condition number of $\bX_{\star}$. Define the ground truth low-rank factors as $\bL_{\star}\coloneqq\bU_{\star}\bSigma_{\star}^{1/2}$ and $\bR_{\star}\coloneqq\bV_{\star}\bSigma_{\star}^{1/2}$, so that $\bX_{\star}=\bL_{\star}\bR_{\star}^{\top}$. Correspondingly, denote the stacked factor matrix as $\bF_{\star}\coloneqq[\bL_{\star}^{\top},\bR_{\star}^{\top}]^{\top}\in\RR^{(n_{1}+n_{2})\times r}$.

Next, we are in need of a right metric to measure the performance of the \texttt{ScaledGD} iterates $\bF_{t}\coloneqq[\bL_{t}^{\top},\bR_{t}^{\top}]^{\top}$. 
Obviously, the factored representation is not unique in that for any invertible matrix $\bQ\in\GL(r)$, one has $\bL\bR^\top=(\bL\bQ)(\bR\bQ^{-\top})^{\top}$. Therefore, the reconstruction error metric needs to take into account this identifiability issue. More importantly, we need a diagonal scaling in the distance error metric to properly account for the effect of pre-conditioning. Taking both considerations together leads to the following error metric
\begin{align}
\dist^{2}(\bF,\bF_{\star})\coloneqq\inf_{\bQ\in\GL(r)}\;\left\Vert (\bL\bQ-\bL_{\star})\bSigma_{\star}^{1/2}\right\Vert _{\fro}^{2}+\left\Vert (\bR\bQ^{-\top}-\bR_{\star})\bSigma_{\star}^{1/2}\right\Vert _{\fro}^{2}.\label{eq:dist}
\end{align}
Correspondingly, we define the optimal alignment matrix $\bQ$ between $\bF$ and $\bF_{\star}$ as 
\begin{align}
\bQ\coloneqq\argmin_{\bQ\in\GL(r)}\;\left\Vert (\bL\bQ-\bL_{\star})\bSigma_{\star}^{1/2}\right\Vert _{\fro}^{2}+\left\Vert (\bR\bQ^{-\top}-\bR_{\star})\bSigma_{\star}^{1/2}\right\Vert _{\fro}^{2},\label{eq:Q_def}
\end{align}
whenever the minimum is achieved. It turns out that for the \texttt{ScaledGD} iterates $\{\bF_{t}\}$, the optimal alignment matrices $\{\bQ_{t}\}$ always exist (at least when properly initialized) and hence are well-defined. The design and analysis of this new distance metric are of crucial importance in obtaining the improved rate of \texttt{ScaledGD}.
In comparison, the previously studied distance metrics (proposed mainly for GD) either do not include the diagonal scaling \cite{ma2019beyond,tu2015low}, or only consider the ambiguity class up to orthonormal transforms \cite{tu2015low}, which fail to unveil the benefit of \texttt{ScaledGD}.  

\subsection{Theoretical Guarantees for Low-Rank Matrix Sensing}

To understand the performance of \texttt{ScaledGD} for low-rank matrix sensing, we adopt a standard assumption on the sensing operator $\cA(\cdot)$, namely the Restricted Isometry Property (RIP). 
\begin{definition}[RIP \cite{recht2010guaranteed}] The linear map $\cA(\cdot)$ is said to obey the rank-$r$ RIP with a constant $\delta_{r}\in[0,1)$, if for all matrices $\bM\in\RR^{n_{1}\times n_{2}}$ of rank at most $r$, one has 
\begin{align*}
(1-\delta_{r})\|\bM\|_{\fro}^{2}\le\|\cA(\bM)\|_{2}^{2}\le(1+\delta_{r})\|\bM\|_{\fro}^{2}.
\end{align*}
\end{definition}

It is well-known that many measurement ensembles satisfy the RIP property \cite{recht2010guaranteed,candes2011tight}. For example, if the entries of $\bA_{i}$'s are composed of i.i.d.~Gaussian entries $\cN(0,1/m)$, then the RIP is satisfied for a constant $\delta_{r}$ as long as $m$ is on the order of $(n_{1}+n_{2})r/\delta_{r}^{2}$. 

With the RIP condition in place, the following theorem demonstrates that \texttt{ScaledGD} converges linearly --- in terms of the new distance metric (cf.~\eqref{eq:dist}) --- at a constant rate as long as the sensing operator $\cA(\cdot)$ has a sufficiently small RIP constant.

\begin{theorem}\label{thm:MS} Suppose that $\cA(\cdot)$ obeys the $2r$-RIP with $\delta_{2r}\le0.02/(\sqrt{r}\kappa)$. If the step size obeys $0<\eta\le2/3$, then for all $t\ge0$, the iterates of the \texttt{ScaledGD} method in Algorithm~\ref{alg:MS} satisfy 
\begin{align*}
\dist(\bF_{t},\bF_{\star})\le(1-0.6\eta)^{t}0.1\sigma_{r}(\bX_{\star}),\quad\mbox{and}\quad\left\Vert \bL_{t}\bR_{t}^{\top}-\bX_{\star}\right\Vert _{\fro}\le(1-0.6\eta)^{t}0.15\sigma_{r}(\bX_{\star}).
\end{align*}
\end{theorem}

Theorem~\ref{thm:MS} establishes that the distance $\dist(\bF_{t},\bF_{\star})$ contracts linearly at a constant rate, as long as the sample size satisfies $m=O(nr^{2}\kappa^{2})$ with Gaussian random measurements \cite{recht2010guaranteed}, where $n\coloneqq\max\{n_{1},n_{2}\}$.
To reach $\epsilon$-accuracy, i.e.~$\|\bL_{t}\bR_{t}^{\top}-\bX_{\star}\|_{\fro}\le\epsilon\sigma_{r}(\bX_{\star})$, \texttt{ScaledGD} takes at most $T=O(\log(1/\epsilon))$ iterations, which is {\em independent} of the condition number $\kappa$ of $\bX_{\star}$. 
In comparison, alternating minimization with spectral initialization (\texttt{AltMinSense}) converges in $O(\log(1/\epsilon))$ iterations as long as $m=O(nr^{3}\kappa^{4})$ \cite{jain2013low}, where the per-iteration cost is much higher requiring solving two linear systems of size $O(mnr)$. On the other end, gradient descent with spectral initialization in \cite{tu2015low} converges in $O(\kappa\log(1/\epsilon))$ iterations as long as $m=O(nr^{2}\kappa^{2})$.
Therefore, \texttt{ScaledGD} converges at a much faster rate than GD at the same sample complexity while requiring a significantly lower per-iteration cost than \texttt{AltMinSense}.

\begin{remark} \cite{tu2015low} suggested that one can employ a more expensive initialization scheme, e.g.~performing multiple projected gradient descent steps over the low-rank matrix, to reduce the sample complexity. By seeding \texttt{ScaledGD} with the output of updates of the form $\bX_{\tau+1}=\cP_{r}\left(\bX_{\tau}-\cA^{*}(\cA(\bX_{\tau})-\by)\right)$ after $T_{0}\gtrsim\max\{\log r,\log\kappa\}$ iterations, where $\cP_r(\cdot)$ is defined in \eqref{eq:rank_r_proj}, \texttt{ScaledGD} succeeds with the sample size $O(nr)$ which is information theoretically optimal.
\end{remark}


\subsection{Theoretical Guarantees for Robust PCA}

Before stating our main result for robust PCA, we introduce the incoherence condition which is known to be crucial for reliable estimation of the low-rank matrix $\bX_{\star}$ in robust PCA~\cite{chen2015incoherence}. 
\begin{definition}[Incoherence]\label{def:incoherence} A rank-$r$ matrix $\bX_{\star}\in\RR^{n_{1}\times n_{2}}$ with compact SVD as $\bX_{\star}=\bU_{\star}\bSigma_{\star}\bV_{\star}^{\top}$ is said to be $\mu$-incoherent if
\begin{align*}
\|\bU_{\star}\|_{2,\infty}\le\sqrt{\frac{\mu}{n_{1}} }\|\bU_{\star}\|_{\fro}=\sqrt{\frac{\mu r}{n_{1}}},\quad\mbox{and}\quad\|\bV_{\star}\|_{2,\infty}\le\sqrt{\frac{\mu}{n_{2}}}\|\bV_{\star}\|_{\fro}=\sqrt{ \frac{\mu r}{n_{2}}}.
\end{align*}
\end{definition}

The following theorem establishes that \texttt{ScaledGD} converges linearly at a constant rate as long as the fraction $\alpha$ of corruptions is sufficiently small.

\begin{theorem}\label{thm:RPCA} Suppose that $\bX_{\star}$ is $\mu$-incoherent and that the corruption fraction $\alpha$ obeys $\alpha\le c/(\mu r^{3/2}\kappa)$ for some sufficiently small constant $c>0$. If the step size obeys $0.1\le\eta\le2/3$, then for all $t\ge0$, the iterates of \texttt{ScaledGD} in Algorithm~\ref{alg:RPCA} satisfy 
\begin{align*}
\dist(\bF_{t},\bF_{\star}) & \le(1-0.6\eta)^{t}0.02\sigma_{r}(\bX_{\star}),\quad\mbox{and}\quad\left\Vert \bL_{t}\bR_{t}^{\top}-\bX_{\star}\right\Vert _{\fro}\le(1-0.6\eta)^{t}0.03\sigma_{r}(\bX_{\star}).
\end{align*}
\end{theorem}

Theorem~\ref{thm:RPCA} establishes that the distance $\dist(\bF_{t},\bF_{\star})$ contracts linearly at a constant rate, as long as the fraction of corruptions satisfies $\alpha\lesssim1/(\mu r^{3/2}\kappa)$.
To reach $\epsilon$-accuracy, i.e.~$\left\Vert \bL_{t}\bR_{t}^{\top}-\bX_{\star}\right\Vert _{\fro}\le\epsilon\sigma_{r}(\bX_{\star})$, \texttt{ScaledGD} takes at most $T=O(\log(1/\epsilon))$ iterations, which is {\em independent} of $\kappa$. 
In comparison, the \texttt{AltProj} algorithm with spectral initialization converges in $O(\log(1/\epsilon))$ iterations as long as $\alpha\lesssim1/(\mu r)$ \cite{netrapalli2014non},
\footnote{\texttt{AltProj} employs a multi-stage strategy to remove the dependence on $\kappa$ in $\alpha$, which we do not consider here. The same strategy might also improve the dependence on $\kappa$ for \texttt{ScaledGD}, which we leave for future work.} where the per-iteration cost is much higher both in terms of computation and memory as it requires the computation of the low-rank SVD of the full matrix. 
On the other hand, projected gradient descent with spectral initialization in \cite{yi2016fast} converges in $O(\kappa\log(1/\epsilon))$ iterations as long as $\alpha\lesssim\min\{1/(\mu r^{3/2}\kappa^{3/2}),1/(\mu r\kappa^{2})\}$.
Therefore, \texttt{ScaledGD} converges at a much faster rate than GD while requesting a significantly lower per-iteration cost than \texttt{AltProj}. In addition, our theory suggests that \texttt{ScaledGD} maintains the incoherence and balancedness of the low-rank factors without imposing explicit regularizations, which is not captured in previous analysis \cite{yi2016fast}.

\subsection{Theoretical Guarantees for Matrix Completion}



To understand the performance of \texttt{ScaledPGD} for low-rank matrix completion, we assume that
$\bX_{\star}$ is $\mu$-incoherent.
\begin{theorem}\label{thm:MC} Suppose that $\bX_{\star}$ is $\mu$-incoherent, the sampling rate satisfies $p\ge C\mu^{2}r^{2}\kappa^{4}\log(n_{1}\vee n_{2})/(n_{1}\wedge n_{2})$ for some sufficiently large constant $C$. Set the projection radius as $B=C_{B}\sqrt{\mu r}\sigma_{1}(\bX_{\star})$ for some constant $C_{B}\ge1.02$. If the step size satisfies $0<\eta\le2/3$, then for all $t\ge0$, with overwhelming probability (i.e.~at least $1-c_{1}(n_{1}\vee n_{2})^{-c_{2}}$), the iterates of \texttt{ScaledPGD} in \eqref{eq:iterates_MC} satisfy
\begin{align*}
\dist(\bF_{t},\bF_{\star})\le(1-0.6\eta)^{t}0.02\sigma_{r}(\bX_{\star}),\quad\mbox{and}\quad\left\|\bL_{t}\bR_{t}^{\top}-\bX_{\star}\right\|_{\fro}\le(1-0.6\eta)^{t}0.03\sigma_{r}(\bX_{\star}).
\end{align*} 
\end{theorem}
\begin{remark} The term $\kappa^{4}$ in the sampling rate comes from the incoherence condition \eqref{eq:cond_MC_2inf-1}: 
\begin{align*}
\sqrt{n_{1}}\|\bL_{t}\bQ_{t}\bSigma_{\star}^{1/2}\|_{2,\infty}\vee\sqrt{n_{2}}\|\bR_{t}\bQ_{t}^{-\top}\bSigma_{\star}^{1/2}\|_{2,\infty}\le \frac{C_{B}}{1-\epsilon}\sqrt{\mu r}\sigma_{1}(\bX_{\star}).
\end{align*}
Using projections, it seems hopeless to further improve the order of $\kappa$. Ideally, we want the following incoherence condition: 
\begin{align*}
\sqrt{n_{1}}\|(\bL_{t}\bQ_{t}-\bL_{\star})\bSigma_{\star}^{1/2}\|_{2,\infty}\vee\sqrt{n_{2}}\|(\bR_{t}\bQ_{t}^{-\top}-\bR_{\star})\bSigma_{\star}^{1/2}\|_{2,\infty}\le\sqrt{\mu r}\sigma_{r}(\bX_{\star}),
\end{align*}
just like what we argued for RPCA. Given that, the sampling rate of local contraction (cf.~Lemma~\ref{lemma:contraction_MC}) does not depend on $\kappa$, while the spectral initialization (cf.~Lemma~\ref{lemma:init_MC}) requires $\kappa^{2}$.
\end{remark}



\subsection{Theoretical Guarantees under General Loss Functions}

In the sequel, we generalize our analysis of \texttt{ScaledGD} to minimize a general loss function in the form of \eqref{eq:problem}, where the update rule of \texttt{ScaledGD} is given by
\begin{align}
\begin{split} \bL_{t+1} &=\bL_{t}-\eta\nabla f(\bL_{t}\bR_{t}^{\top})\bR_{t}(\bR_{t}^{\top}\bR_{t})^{-1},\\
 \bR_{t+1} &=\bR_{t}-\eta\nabla f(\bL_{t}\bR_{t}^{\top})^{\top}\bL_{t}(\bL_{t}^{\top}\bL_{t})^{-1}.
\end{split}\label{eq:scaledGD_GL}
\end{align}

Two important properties of the loss function $f(\cdot):\RR^{n_{1}\times n_{2}}\mapsto\RR$ play a key role in the analysis. 
\begin{definition}[Restricted smoothness]\label{def:restricted_smooth} A differentiable function $f(\cdot):\RR^{n_{1}\times n_{2}}\mapsto\RR$ is said to be rank-$r$ restricted $L$-smooth for some $L>0$ if 
\begin{align*}
f(\bX_{2})\le f(\bX_{1})+\langle\nabla f(\bX_{1}),\bX_{2}-\bX_{1}\rangle+\frac{L}{2}\|\bX_{2}-\bX_{1}\|_{\fro}^2,
\end{align*}
for any $\bX_{1},\bX_{2}\in\RR^{n_{1}\times n_{2}}$ with rank at most $r$.
\end{definition}
\begin{definition}[Restricted strong convexity]\label{def:restricted_strongly_convex} A differentiable function $f(\cdot):\RR^{n_{1}\times n_{2}}\mapsto\RR$ is said to be rank-$r$ restricted $\mu$-strongly convex for some $\mu\ge0$ if 
\begin{align*}
f(\bX_{2})\ge f(\bX_{1})+\langle\nabla f(\bX_{1}),\bX_{2}-\bX_{1}\rangle+\frac{\mu}{2}\|\bX_{2}-\bX_{1}\|_{\fro}^2,
\end{align*}
for any $\bX_{1},\bX_{2}\in\RR^{n_{1}\times n_{2}}$ with rank at most $r$. When $\mu=0$, we simply say $f(\cdot)$ is rank-$r$ restricted convex.
\end{definition}
Further, when $\mu>0$, define the condition number of the loss function $f(\cdot)$ over rank-$r$ matrices as
\begin{align} 
\kappa_{f}\coloneqq L/\mu,\label{eq:kappa_f}
\end{align}
which plays an important role in the convergence analysis. 
Encouragingly, many problems can be viewed as a special case of optimizing this general loss \eqref{eq:scaledGD_GL}, including but not limited to:
\begin{itemize}
\item {\em low-rank matrix factorization}, where the loss function $f(\bX)=\frac{1}{2}\|\bX-\bX_{\star}\|_{\fro}^2$ in \eqref{eq:loss_MF} satisfies $\kappa_{f}=1$;
\item {\em low-rank matrix sensing}, where the loss function $f(\bX)=\frac{1}{2}\|\cA(\bX-\bX_{\star})\|_{2}^2$ in \eqref{eq:loss_MS} satisfies $\kappa_{f}\approx 1$ when $\cA$ obeys the rank-$r$ RIP with a sufficiently small RIP constant;
\item {\em quadratic sampling}, where the loss function $f(\bX)=\frac{1}{2}\sum_{i=1}^{m}|\langle \ba_i\ba_i^{\top}, \bX-\bX_{\star} \rangle|^2$ satisfies restricted strong convexity and smoothness when $\ba_i$'s are i.i.d.~Gaussian vectors for sufficiently large $m$ \cite{sanghavi2017local,li2018nonconvex};
\item {\em exponential-family PCA}, where the loss function $f(\bX)=-\sum_{(i,j)} \log p(\bY_{i,j}|\bX_{i,j})$, where $p(\bY_{i,j}|\bX_{i,j})$ is the probability density function of $\bY_{i,j}$ conditional on $\bX_{i,j}$, following an exponential-family distribution such as Bernoulli and Poisson distributions. The resulting loss function satisfies restricted strong convexity and smoothness with a condition number $\kappa_{f}>1$ depending on the property of the specific distribution \cite{gunasekar2014exponential,lafond2015low}.
\end{itemize}

Indeed, the treatment of a general loss function brings the condition number of $f(\cdot)$ under the spotlight, since in our earlier case studies $\kappa_{f}\approx1$. Our purpose is thus to understand the interplay of two types of conditioning numbers in the convergence of first-order methods. For simplicity, we assume that $f(\cdot)$ is minimized at the ground truth rank-$r$ matrix $\bX_{\star}$.\footnote{In practice, due to the presence of statistical errors due to noise, the minimizer of $f(\cdot)$ might be only approximately low-rank, to which our analysis can be extended in a straightforward fashion.} The following theorem establishes that as long as properly initialized, then \texttt{ScaledGD} converges linearly at a constant rate. 

\begin{theorem}\label{thm:GL} Suppose that $f(\cdot):\RR^{n_{1}\times n_{2}}\mapsto\RR$ is rank-$2r$ restricted $L$-smooth and $\mu$-strongly convex, of which $\bX_{\star}$ is a minimizer, and that the initialization $\bF_{0}$ satisfies $\dist(\bF_{0},\bF_{\star})\le0.1\sigma_{r}(\bX_{\star})/\sqrt{\kappa_{f}}$. If the step size obeys $0<\eta\le0.4/L$, then for all $t\ge0$, the iterates of \texttt{ScaledGD} in \eqref{eq:scaledGD_GL} satisfy
\begin{align*}
\dist(\bF_{t},\bF_{\star})\le(1-0.7\eta\mu)^{t}0.1\sigma_{r}(\bX_{\star})/\sqrt{\kappa_{f}},\quad\mbox{and}\quad\left\Vert \bL_{t}\bR_{t}^{\top}-\bX_{\star}\right\Vert _{\fro}\le(1-0.7\eta\mu)^{t}0.15\sigma_{r}(\bX_{\star})/\sqrt{\kappa_{f}}.
\end{align*} 
\end{theorem}

Theorem~\ref{thm:GL} establishes that the distance $\dist(\bF_{t},\bF_{\star})$ contracts linearly at a constant rate, as long as the initialization $\bF_{0}$ is sufficiently close to $\bF_{\star}$.
To reach $\epsilon$-accuracy, i.e.~$\|\bL_{t}\bR_{t}^{\top}-\bX_{\star}\|_{\fro}\le\epsilon\sigma_{r}(\bX_{\star})$, \texttt{ScaledGD} takes at most $T=O(\kappa_{f}\log(1/\epsilon))$ iterations, which depends only on the condition number $\kappa_{f}$ of $f(\cdot)$, but is independent of the condition number $\kappa$ of the matrix $\bX_{\star}$. In contrast, prior theory of vanilla gradient descent \cite{park2018finding} requires $O(\kappa_{f}\kappa\log(1/\epsilon))$ iterations, which is worse than our rate by a factor of $\kappa$.  
 

